From Attack Tree to Model Checker: Binding CAPEC Patterns to Verify Robotic System Security

Security-minded verification of autonomous and robotic systems presupposes an attacker, yet the path from a threat catalogue to a checkable attacker model is still traversed by hand. This research preview presents the theory and construction of a pipeline that mechanises it. Each leaf of an attack tree is mapped to a CAPEC attack pattern and written in first-order logic as a rule: the attacker's prerequisites imply the attack's effect. Casting the pattern as such a rule is what makes it operational - its variables can be bound to a specific system's parts, and its prerequisites can then be tested against that system under a chosen configuration of security controls. Binding is our means of verifying whether a system is vulnerable to a given attack: from a bound pattern we derive an attacker model, turn its effect into a temporal-logic property, and check that property against the system with and without a countermeasure, reporting the control that defeats the attack. We describe the signature, schemas, profiles for approach, and explore how CAPEC can support reasoning about robotics security.

==> eptcsdata.tex <==
\providecommand{\firstpage}{154}
\providecommand{\publicationstatus}{Matt Luckcuck, Maike Schwammberger, \& Akhila Bairy (Eds.):\\
Eighth International Workshop on Formal Methods\\
for Autonomous Systems (FMAS 2026)\\
EPTCS 457, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.457.11}{10.4204/EPTCS.457.11}}
\pdfoutput=1

